Fast Optimization with Zeroth-Order Feedback in Distributed, Multi-User MIMO Systems

In this paper, we develop a gradient-free optimization methodology for efficient resource allocation in Gaussian MIMO multiple access channels. Our approach combines two main ingredients: (i) an entropic semidefinite optimization based on matrix exponential learning (MXL); and (ii) a one-shot gradient estimator which achieves low variance through the reuse of past information. This novel algorithm, which we call gradient-free MXL algorithm with callbacks (MXL0$^{+}$), retains the convergence speed of gradient-based methods while requiring minimal feedback per iteration$-$a single scalar. In more detail, in a MIMO multiple access channel with $K$ users and $M$ transmit antennas per user, the MXL0$^{+}$ algorithm achieves $\epsilon$-optimality within $\text{poly}(K,M)/\epsilon^2$ iterations (on average and with high probability), even when implemented in a fully distributed, asynchronous manner. For cross-validation, we also perform a series of numerical experiments in medium- to large-scale MIMO networks under realistic channel conditions. Throughout our experiments, the performance of MXL0$^{+}$ matches$-$and sometimes exceeds$-$that of gradient-based MXL methods, all the while operating with a vastly reduced communication overhead. In view of these findings, the MXL0$^{+}$ algorithm appears to be uniquely suited for distributed massive MIMO systems where gradient calculations can become prohibitively expensive.

==> App-Proofs.tex <==
%----------------------------------------------------------------------
%%% APP: PROOFS
%----------------------------------------------------------------------
% !TEX root = ./Supplement.tex


These are the proofs.

==> SPSA.tex <==




==> Tables/Related-old.tex <==
%----------------------------------------------------------------------
%%% PARAMETERS
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\scshape
\begin{tabular}{llccccc}
\textbf{\scshape Algorithm \qquad[source]}
	&\textbf{Feedback}
	&\textbf{Convergence}
	&\textbf{Conv. Speed}
	&\textbf{Distributed}
	&\textbf{Off. Overhead}
	&\textbf{Iter. Overhead}
	\\
\hline
\hline
\acs{IWF}
	\hfill
	\cite{YRBC04}
	&full matrix
	&\checkmark
	&$\bigoh(\kk\log(1/\eps))$
	&no
	&$\bigoh(\mm\nn)$ 
	&$\bigoh(\nn^{2})$
	\\
\hline
\acs{SWF}
	\hfill
	\cite{SPB06}
	&full matrix
	&no
	&\textemdash
	&\checkmark
	&$\bigoh(\kk\mm\nn)$
	&$\bigoh(\nn^{2})$
	\\
\hline
\acs{IWMMSE}
	\hfill
	\cite{CADC08,SRLH11}
	&full matrix
	&\checkmark
	&\textemdash
	&\checkmark
	&$\bigoh(\kk\mm\nn)$
	&$\bigoh(\nn^{2})$
	\\
\hline
\acs{MXL}
	\hfill
	\cite{MM16}
	&full matrix (imp.)
	&\checkmark
	&$\bigoh(1/\eps^{2})$
	&\checkmark
	&$\bigoh(\kk\mm\nn)$
	&$\bigoh(\nn^{2})$
	\\
\hline
\hline
\acs{MXL0}
	\hfill
	[this paper]
	&scalar
	&\checkmark
	&$\bigoh(1/\eps^{4})$
	&\checkmark
	&none
	&$\bigoh(1)$
	\\
\hline
\acs{MXL+}
	\hfill
	[this paper]
	&scalar
	&\checkmark
	&$\bigoh(1/\eps^{2})$
	&\checkmark
	&none
	&$\bigoh(1)$
	\\
\hline
\end{tabular}

==> Thanks.tex <==
%----------------------------------------------------------------------
%%% THANKS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex
%
%

\VB{Why we need this if we put the projects on the first page? Also, I guess all of us can acknowledge  ORACLESS.}

(...)

P.~Mertikopoulos was partially supported by
the French National Research Agency (ANR) grant
ORACLESS (ANR\textendash 16\textendash CE33\textendash 0004\textendash 01).

